Topological analysis of the power grid and mitigation strategies against cascading failures

This paper presents a complex systems overview of a power grid network. In recent years, concerns about the robustness of the power grid have grown because of several cascading outages in different parts of the world. In this paper, cascading effect has been simulated on three different networks, the IEEE 300 bus test system, the IEEE 118 bus test system, and the WSCC 179 bus equivalent model, using the DC Power Flow Model. Power Degradation has been discussed as a measure to estimate the damage to the network, in terms of load loss and node loss. A network generator has been developed to generate graphs with characteristics similar to the IEEE standard networks and the generated graphs are then compared with the standard networks to show the effect of topology in determining the robustness of a power grid. Three mitigation strategies, Homogeneous Load Reduction, Targeted Range-Based Load Reduction, and Use of Distributed Renewable Sources in combination with Islanding, have been suggested. The Homogeneous Load Reduction is the simplest to implement but the Targeted Range-Based Load Reduction is the most effective strategy.

==> PG_bib.tex <==
@InProceedings{MKA:07,
author = {M.Anghel and K.A. Werley and A.E. Motter},  
title = {{Stochastic Model for Power Grid Dynamics}},
booktitle = {{40th Hawaii International Conference on System Sciences}}, 
year = {2007},
}

@unpublished{planetlab,
  TITLE ={\url{http://www.planet-lab.org}},
}

@unpublished{SD:04,
TITLE = {\url{ http://www.sciencedaily.com/releases/2004/09/040903090113.htm}}, 
}

@InProceedings{NB:09,
author = {N.Bhatt and et al},  
title = {Assessing Vulnerability to Cascading Outages},
booktitle = {{Power Systems Conference and Exposition}},
month = {March},
year = {2009},
}


@InProceedings{RPRV:04,
author = {R.Kinney and P.Crucitti and R.Albert and V.Latora},  
title = {{Modeling Cascading Failures in the North American Power Grid}},
month = {October},
year = {2004},
}

@InProceedings{BDIA:00,
author = {B.A.Carreras and D.E.Newman and I.Dolrou and A.B.Poole},  
title = {{Proceedings of the Hawaii International Conference on System Sciences(unpublished)}},
year = {2000},
}


@InProceedings{MBV:00,
author = {M.L. Sachtjen and B.A.Carreras and V.E.Lynch},  
title = {{Phys. Rev. E61, 4877}},
year = {2000},
}

@article{JR:03,
author = {J.Glanz and R.Perez-Pena},  
title = {{90 Seconds That Left Tens of Millions of people in the Park}}, 
booktitle = {New York Times}}, 
month={August}, 
year = {2003},

}

@InProceedings{AR:1999,
author = {A.L.Barabasi and R.Albert},  
title = {{Emergence of Scaling in Random Networks}},
booktitle = {{Science 286,509}},
year = {1999},
}


@InProceedings{AY:00,
author = {A.E.Motter and Y.C.Lai},  
title = {{Phys. Rev. E 66, 065102(R)}},
year = {2000},
}

@InProceedings{PVM:04,
author = {P.Crucitti and V.Latora and M.Marchiori},  
title = {{A Topological Analysis of the Italian 
Electric Power Grid}},
year = {2004},
}


@InProceedings{LAMH:00,
author = {L.A.N Amaral and A.Scala and M.Bartehelemy and H.E.Stanley},  
title = {{Proc. Natl.Acad.Sci.USA 97(2000)11149}},
year = {2000},
}

@unpublished {WAS,
TITLE = {\url{http://www.ee.washington.edu/research/pstca/index.htm}},
}


@InProceedings{NERC:05,
author = {Evaluation of Criteria, Methods, and Practices used for System Design, Planning, and Analysis Response to NERC Blackout Recommendation 13c 

[Online]},
year = {2005},
title = {\url{http://www.nerc.com/docs/pc/tis/}}
}


@BOOK{BR:88,
AUTHOR = {B.R.Gungor},
TITLE = {{Power Systems}},
PUBLISHER = {Technology Publications},
year={1988}
} 


@unpublished{EIA,
TITLE = {\url{http://www.eia.doe.gov/cneaf/}},
}


@InProceedings{KD:09,
author = {K.Davis}, 
title = {{Smart Talk Directly From the DOE}},
booktitle = {{T\&D}},
pages= {30-34},
month = {January}, 
year = {2009},
}

@InProceedings{JSK:09,
author =  {J.S.Katz}, 
title = {{Smart Talk Directly From the DOE}},
booktitle = {{T\&D}},
pages= {30-34},
month = {January}, 
year = {2009},
}

@InProceedings{JPC:09,
author = {J.P.Crane}, 
title = {{Illinois Smart Grid Work Advances at National, State Levels}},
booktitle = {{T\&D}},
pages= {40-42},
month = {January}, 
year = {2009},
}


@InProceedings{MBPE:07,
author = {E.Muljadi and C.P.Butterfield and Brian Parsons and Abraham Ellis}, 
title = {{Effect of variable speed wind turbine generator on stability of a weak grid (Author abstract)}},
booktitle = {{IEEE Transactions on Energy Conversion 22.1}},
month = {March}, 
year = {2007},
}


@InProceedings{JMC:06,
author = {J.Carrasco and et al.}, 
title = {{Power-Electronic Systems for the Grid Integration of Renewable Energy}},
booktitle = {{Industrial Electrinics, IEEE Transactions}},
month = {June}, 
year = {2006},
}


@InProceedings{TLG:01,
author = {T.Ackermann and G.Andersson and L.Soder}, 
title = {{Distributed Generation : a Definition}},
booktitle = {{Electrical Power Systems Research(ELSVIER)}}, 
year = {2001},
}


@InProceedings{DJS:07,
author = {D.J.Swider}, 
title = {{Compressed air energy storage in an electricity system with significant wind power generation(Author abstract)}},
booktitle = {{IEEE Transactions on Energy Conversion}},
month = {March},
year = {2007},
}


@unpublished{BER,
TITLE = {\url{http://www.bergey.com}},
}
 

@InProceedings{ASB:08, 
author = {A.Faza and S.S.Sarvestani and B.McMillin}, 
title = {{The Advanced Electric Power Grid : Complexity Reduction Techniques for Reliability Modeling}},
booktitle = {{Lecture Notes on Computer Science}},
month = {September},
year = {2008},
}

@InProceedings{MMFAS:07,
author = {{McMillin and M.Bruce and Faza and A.Z.Salem and S.S. Sarvestani}}, 
booktitle = {{Computer Safety, Reliability and Security}},
year = {2007},
}
